Multi-View Multi-Task Representation Learning for Mispronunciation Detection

The disparity in phonology between learner's native (L1) and target (L2) language poses a significant challenge for mispronunciation detection and diagnosis (MDD) systems. This challenge is further intensified by lack of annotated L2 data. This paper proposes a novel MDD architecture that exploits multiple `views' of the same input data assisted by auxiliary tasks to learn more distinctive phonetic representation in a low-resource setting. Using the mono- and multilingual encoders, the model learn multiple views of the input, and capture the sound properties across diverse languages and accents. These encoded representations are further enriched by learning articulatory features in a multi-task setup. Our reported results using the L2-ARCTIC data outperformed the SOTA models, with a phoneme error rate reduction of 11.13% and 8.60% and absolute F1 score increase of 5.89%, and 2.49% compared to the single-view mono- and multilingual systems, with a limited L2 dataset.

==> articulatory_sec.tex <==
\section{Articulatory Features}
Articulatory features are the physical properties of speech sounds that are used to distinguish them from each other. The four main articulatory features are place of articulation, manner of articulation, high-low, and front-back. Each articulatory feature is abstracted into several classes, which indicate distinct behaviors \cite{scharenborg2007towards}. 

\begin{itemize}
    \item \textbf{Place of articulation} refers to the position of the articulators (the tongue, lips, teeth, and palate) in the vocal tract when a speech sound is produced. 
    \item  \textbf{Manner of articulation} refers to the way in which the airstream is obstructed or modified in the vocal tract when a speech sound is produced.
    \item  \textbf{High-low} refers to the position of the tongue in the vocal tract when a speech sound is produced. 
    \item \textbf{Front-back} refers to the position of the tongue in the vocal tract when a speech sound is produced. 
\end{itemize}

These four articulatory features are used to distinguish between all the different speech sounds in the world's languages. For example, the English consonants /p/, /t/, and /k/ are all produced with the same place of articulation (bilabial), but they differ in their manner of articulation (plosive, fricative, and affricate). The English vowels /i/, /e/, and /æ/ are all produced with the same manner of articulation (high), but they differ in their position of articulation (front, central, and back).

As presented in Table 1, this feature space offers a structured framework for encoding and analyzing articulatory characteristics associated with phonemes, facilitating a comprehensive understanding of speech production. 


\begin{table}[htbp]
  \centering
  \setlength{\tabcolsep}{6pt} % Adjust the spacing between columns
  \renewcommand{\arraystretch}{1.2} % Adjust the spacing between rows
  \begin{tabular}{cp{3cm}cc} % Three columns with fixed width
    \hline
    \textbf{Stream} & \textbf{Classes} & \textbf{Cardinality} & \textbf{Code} \\
    \hline
    \hline
    Manner & vowel, stop, fricative, retroflex, approximant, nasal, sricative & 7 & AF_M\\
    \hline
    Place & blibial, alveolar, dental, labiodental, velar, nil & 7 & AF_P \\
    \hline
    High-low & low, mid, high, nil, & 4 & AF_{HL}\\
    \hline
    Fr-back & front, central, back, nil, & 4 & AF_{FR}\\
    \hline
  \end{tabular}
  \caption{The articulatory features spaces}
\end{table}

Thanks to the distinctive information included in articulatory features, the use of articulatory features in MDD is helpful in distinguishing phonemes, especially for some confusing phonemes pairs. Thus in this paper, we employ the articulatory features to boost the state-of-the-art approaches to MDD.












\subsection{Pre-trained Speech Encoders}
\paragraph*{Monolingual Encoder Wav2vec2-base}: Wav2vec2-base\footnote{https://huggingface.co/facebook/wav2vec2-base} comprises Convolutional Neural Network (CNN) and Transformer layers. The CNNs serve as a feature extractor that converts the input audio waveform $X$ into a latent representation $Z$. Prior to being fed into the Transformer layers, $Z$ undergoes random masking, where a certain portion is masked. The Transformer layers contextualize $Z$ and produce the contextualized representation $C$. The unmasked latent representation $Z$ is further discretized into $Q$ using a learnable codebook. During pre-training, Wav2vec2.0-base is trained using Contrastive Loss only on English Data, which aims to differentiate the true underlying discretized representation $q^+$ for each masked time step $t$ from those at other masked positions ($q^-$), based on the contextualized representation $c_t$. The complete Semi-Supervised Learning (SSL) loss is a weighted sum of the Contrastive Loss and a codebook diversity loss \cite{baevski2020wav2vec}.

\paragraph*{Multilingual Encoder XLS-R-53 \cite{conneau2020unsupervised}:}

The XLS-R-53\footnote{https://huggingface.co/facebook/wav2vec2-large-xlsr-53} model is a pre-trained wav2vec2.0 \cite{baevski2020wav2vec} model that consists of 53 languages and uses 56,000 hours of speech data for pre-training. The multilingual pre-trained XLS-R-53 model also follows the same architecture as the wav2vec2.0 model. It uses a CNN-based encoder network to encode the raw audio sample and a transformer-based context network to build context representations over the entire latent speech representation. The encoder network consists of $7$ blocks of temporal convolution layers with $512$ channels, and the convolutions in each block have strides and kernel sizes that compress about $25$ms of $16$kHz audio every $20$ms. The context network consists of $24$ blocks with model dimension $1024$, inner dimension $4096$, and $16$ attention heads. 

% The XLS-R-53 model is a pre-trained wav2vec2.0 model that consists of 53 languages speech data for pre-training. The XLS-R-53 model also follows the same architecture as the wav2vec2.0 model. It uses a CNN-based encoder network to encode the raw audio sample and a transformer-based context network to build context representations over the entire latent speech representation. The encoder network consists of $7$ blocks of temporal convolution layers with $512$ channels, and the convolutions in each block have strides and kernel sizes that compress about $25$ms of $16$kHz audio every $20$ms. The context network consists of $24$ blocks with model dimension $1024$, inner dimension $4096$, and $16$ attention heads. 

% \textbf{Monolingual speech encoder wav2vec2-base}:
% \text
% \newline
% \textbf{Contrastive Predictive Coding (CPC) \cite{oord2018representation}:}
% CPC aims to distinguish the latent representation from a series of distractors sampled from other masked time steps, given the contextual representation conditioned on the masked $Z$. CPC provides an easier learning objective. Before contrast training, the unmasked $Z$ is discretized in continuous space using the vector quantization module $VQ: Z \rightarrow Q$. This process converts the representations into a finite number of entries. Considering the discrete nature of phonetic units, $VQ$ learns meaningful speech representations that correspond to underlying speech units without supervision.

% The XLS-R model is a pre-trained wav2vec2.0 \cite{baevski2020wav2vec} model that consists of 53 languages and uses 56,000 hours of speech data for pre-training. The XLS-R model also follows the same architecture as the wav2vec2.0 model. It uses a CNN-based encoder network to encode the raw audio sample and a transformer-based context network to build context representations over the entire latent speech representation.

% During pre-training, a certain proportion of consecutive time steps in the latent representation $Z$ are masked, and contrastive predictive coding (CPC) is performed. CPC aims to distinguish the latent representation from a series of distractors sampled from other masked time steps, given the contextual representation conditioned on the masked $Z$. Unlike the autoregressive predictive coding (APC) method that attempts to reconstruct the high-dimensional signal itself, CPC provides an easier learning objective. Before contrast training, the unmasked $Z$ is discretized in continuous space using the vector quantization module $VQ: Z \rightarrow Q$. This process converts the representations into a finite number of entries. Considering the discrete nature of phonetic units, VQ learns meaningful speech representations that correspond to underlying speech units without supervision. The authors report that the discrete representations learned are related to phonemes. The quantization module employs two codebooks with 320 entries each. All the selected discrete entries are concatenated and used in the contrast training task. We assume that these learned general representations could be valuable for Mispronunciation Detection and Diagnosis (MDD) tasks.



% We provide a detailed description of the architecture, including the concatenation of the feature representations, the integration of a projection layer, and the incorporation of separate blocks for phoneme sequence prediction and AF sequence prediction. This section serves as a comprehensive exploration of the architecture behind our multi-view approach, highlighting its potential in advancing the field of audio analysis and prediction.

% In this paper, we propose a novel multi-view approach for audio analysis, specifically focusing on the task of speech encoding and prediction. Our method aims to leverage the complementary strengths of two powerful speech encoders, namely XLS-R and wav2vec-base. By combining these encoders, we obtain two distinct feature representations of dimensions 1024 and 768, respectively. These representations capture different aspects of the input audio and provide a more comprehensive view of the speech signal. To further enhance the predictive capabilities of our model, we concatenate these feature representations and pass them through a multi-task framework. Within this framework, the concatenated features are first processed by a projection layer, which helps to capture important relationships between the two representations. Subsequently, the transformed features are fed into two distinct blocks: a CTC (Connectionist Temporal Classification) block for phoneme sequence prediction and another block for selected articulatory feature (AF) sequence prediction. This multi-view approach capitalizes on the combined power of XLS-R and wav2vec-base encoders, effectively integrating their unique representations to improve the accuracy and robustness of speech analysis tasks.


==> tables.tex <==
\begin{table*}[!ht]
\centering
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{p{4cm}p{3cm}p{3cm}cccc}
\hline
\textbf{Models} & \textbf{Pre-training/Fine-tuning} & \textbf{L2-ARCTIC} (\#Train/\#Test) & \textbf{R} & \textbf{P} & \textbf{F1} & \textbf{PER}\\ \hline
\hline
\textbf{GOP \cite{DNN_3}} & Librispeech / - & - / 6 & 69.97\% & 32.54\% & 44.42\% & -  \\  \hline
\textbf{CNN-RNN-CTC \cite{non_ASR}} & - / TIMIT & 12 / 6 & 74.78\% & 36.76\% & 49.29\% & - \\  \hline
% \textbf{Mask-CTC \cite{yan2023peppanet}} & - / TIMIT & 12 / 6 & 51.71\% & 52.32\% & 52.01\% & - \\  \hline
\textbf{APL-2 \cite{ye2022approach}} & - / TIMIT & 12 / 6 & 54.49\% & 52.79\% & 53.62\% & - \\ \hline
\textbf{Wav2vec2 + Momentum labeling \cite{yang2022improving}} & - / UTD-4Accents & 18 / 6 & 51.20\% & 60.39\% & 55.42\% & 14.36\%  \\ \hline
% \textbf{CTC-ATTN \cite{yan2020end}} & - / TIMIT & 18 / 4 & 70.28\% & 46.57\% & 56.02\% & - \\  \hline
\textbf{Text-CTC-ATTN \cite{fu2021full}} & - / TIMIT & 12 / 6 & 56.12\% & 56.04\% & 56.08\% & 15.58\% \\  \hline
\textbf{Peppanet \cite{yan2023peppanet}} & - / TIMIT &  15 / 6 & 64.53\% & 51.38\% & 56.81\% & - \\ \hline
\textbf{Wav2vec2-960h + Momentum labeling \cite{yang2022improving}} & Librispeech / UTD-4Accents & 18 / 6 & 54.16\% & 58.30\% & 56.16\% & 14.69\%  \\ \hline
\textbf{RNN-T MDD \cite{zhang2023phonetic}} & - / TIMIT & 12 / 6 & 57.2\% & 60.1\% & 58.6\% & 15.73\%  \\  \hline
\textbf{Joint MDD-Align* \cite{lin2022phoneme}} & - / TIMIT & 18 / 6 & 53.31\% & 77.12\% & 63.04\% & - \\  \hline\hline

\cline{1-7}
\multicolumn{7}{c}{\textbf{Our Results}} \\ 
\cline{1-7}

\textbf{Wav2vec2-base} & - & 12 / 6 & 53.90\% & 54.94\% & 54.42\% & 15.91\% \\
\hline
\textbf{MT Wav2vec2-base} & - & 12 / 6 & 54.05\% & 58.30\% & 56.10\% & 14.60\% \\
\hline
\textbf{XLS-R-53} & - & 12 / 6 & 58.93\% & 56.76\% & 57.82\% & 15.48\% \\ \hline
\textbf{MT XLS-R-53} & - & 12 / 6 & 59.17\% & 56.74\% & 57.89\% & 15.46\% \\ \hline 
\textbf{proposed MV-MT-woCNN} & - & 12 / 6 & 58.19\% & 60.43\% & 59.29\% & 14.33\% \\  \hline

		
\textbf{proposed MV-MT-All} & - & 12 / 6 &  56.63\% & 61.04\% & 58.75\% & 14.85\% \\  \hline
\textbf{Proposed MV-MT} & - & 12 / 6 & 59.23\% & 61.43\% & 60.31\% & \textbf{14.13\%} \\  \hline

\end{tabular}
\caption{Experimental results of different methods on
mispronunciation detection}
\title{res2}
\end{table*}

==> tmp.tex <==

The proposed framework leverages learned representation from monolingual and multilingual pre-trained speech encoders, as an input to the mispronunciation detection (MD) model and fine-tuned it by adding multiple auxiliary tasks -- classifying different articulatory feature (AFs) sets that aren't utilized effectively. The underlying assumption is this ensemble of encoders and auxiliary tasks provides a unique `view' of the learners' input signal.  The multi-view representation of the learner's speech helps the model to learn phonetic properties that are either distinct to the target language or shared across multiple languages,  %, by bringing together speech representation learned in monolingual and multilingual settings. %by learner's native language.
while with multi-task approach, the model learns different dimensions of the input signal, allowing further disentanglement of phonetic properties based on properties of speech production. In contrast to the previous MD framework with frame-level phoneme information along with reference text and boundary information \cite{lin2022phoneme}, our proposed framework learns a shared phonetic representation using different types of views -- monolingual, multilingual, AFs -- of the same input signal. 

% Current leading mispronunciation detection and diagnosis (MDD) systems achieve promising performance via end-to-end phoneme recognition.

% This paper proposes novel approaches to mispronunociation detection and diagnosis on second language leraners speech using arcticulatory features. The articulatory fetaures in MDD is helpful in distinguishing phonemes. we use Wav2vec 2.0 as our SSL model and fine-tune it using original labeled L2 speech samples. Automatic spoken language assessment often operates within a regime whereby only a limited quantity of training data is available. This paper applies multi-task learning to spoken language assessment, by assessing two different forms of target learning. C-Wav2vec.2, castcated wav2vec with additional 4 tasks. and sequential learning with two tasks wav2vec.2.0. Compared with baselines, a 11.12\%, 8.23\%, phoneme reduction error rate has been seen using those two multi-stask setting. We showed that using artculotry features in a multitask setting, we can prune the encoder of wav2vec2.0 up to 65\% of encoder layers, by still ahcieving comparable results with state-of-art models. the multitask setting with articulatory features in this case has achieved an imporvement of  

% In this paper, in order to utilize articulatory features in the end-to-end structure,  the model achieves a fully end-to-end system by aligning the audio with the phoneme sequences of the prior text inside the model through the attention mechanism.

% Specifically, we use Wav2vec 2.0 as our SSL model, and fine-tune it using original labeled L2 speech samples

% The paper is about mispronunciation detection and diagnosis, by making use of pre-trained self-supervised models wav2vec. There are many research venues that focuses on on the use of those large self-supervised model, and finetune them on phoneme recognition task. promising results has been seen using XLSR, and using wav2vec-base with momentum with 2 percent imporvment in score. In this paper, we showed another aspect of how to use wav2vec using articulatory features as a target in a multi task setting. 

% This papers focus on the use of articulatory features in a mutlitask 

% Automatic spoken language assessment is a challenging task, especially for second language learners (L2 learners). One of the key challenges in ASLA is mispronunciation detection, which is the identification of errors in pronunciation. Articulatory features are helpful in distinguishing phonemes, which is a key component of mispronunciation detection. In this paper, we propose novel approaches to mispronunciation detection and diagnosis in L2 speech using articulatory features in a multi-task setting. We use Wav2vec 2.0 as our acoustic encoder model and fine-tune it using original labeled L2 speech samples. We also apply multi-task learning (MTL) to ASLA, by assessing two different forms of targets: (1) C-Wav2vec2.0, which is a cascaded Wav2vec 2.0 model for phoneme sequence recongition, and predictiing sequence of four acticulatory features, and Seq-Wav2vec2.0, which a sequential learning model for phoneme recongition and artculorty features. We compare our proposed methods with baseline methods on a publicly available dataset L2-Arctic. Our results show that the proposed methods can achieve significant improvements in mispronunciation detection and diagnosis,  We also show that using articulatory features in an MTL setting can further improve the performance of the proposed methods. Our proposed methods achieved a 11.12\% and 8.23\% phoneme reduction error rate respectively using the two proposed MTL settings. We pruned the encoder of Wav2vec 2.0 by removing 2/3 of the encoder layers. This resulted in a smaller model that was still able to achieve comparable results with state-of-the-art models using the proposed MTL settings with articulatory features. In fact, the pruned model with articulatory features achieved an improvement achieved an improvement of 24.22\% and 18.38\% in phoneme reduction error rate, respectively.

% which achieved a 12.24\% and 9.23\% phoneme reduction error rate. We also showed that using articulatory features in an MTL setting can further improve the performance of the proposed methods. In this case, the MTL setting with articulatory features 


% In our multi-view setting, we leverage both monolingual and multilingual features to improve the phoneme distinction. The choice of incorporating monolingual features stems from the need to differentiate between phonemes within a language due to the sparse production by various speakers accents. On the other hand, the multilingual encoder provides valuable insights into phoneme representations across different languages and accents, enriching the overall phoneme presentation. By combining these views, our framework benefits from the complementary information offered by each view, enhancing the accuracy of phoneme distinction and representation.

% . However, learning these contrasting phonetic representations requires a large amount of annotated L2 data, which is a big obstracle. Therefore
% is one of the primary factors affecting the performance of mispronunciation detection and diagnosis (MDD) models. Learning the  


% L1 and L2 is a key reason for pronunciation errors.
% The native and non-native phonetic variation is one of the main challenges in pronunciation errors.
% Obtaining L2 
% \textcolor{red}{We present a novel method for detecting mispronunciations that incorporates a multi-view and multi-task approach.  Our method combines multilingual and monolingual pre-trained models within a multi-task framework. By incorporating articulatory features as auxiliary tasks for L2 phoneme sequence recognition, we improve the differentiation between phonemes. Furthermore, the integration of both multilingual and monolingual features enhances the accuracy of predicting phoneme sequences. Our methodology demonstrates the effectiveness of these combined techniques, pushing the boundaries of existing methods and offering promising prospects for more accurate mispronunciation detection. In our study, the multi-view multi-task model achieved a 11.13\% and 8.6\% phoneme error rate reduction compared to the monolingual and multilingual proposed models, resulting in phoneme error rate of 14.13\%, and F1-score of 60.31\%.}

% Additionally, the proposed multi-view multi-task setting resulted in a 7.12\% phoneme error rate reduction with an improvement of 2.5\% in F1-measure.


% This research paper introduces an innovative approach to detect mispronunciations by utilizing multi-view and multi-task methodology. The approach leverages both multilingual and monolingual pre-trained models in a multi-task framework, incorporating articulatory features as auxiliary tasks to L2 phoneme sequence recognition.

% By treating articulatory features as auxiliary tasks and combining multilingual and monolingual features, our approach achieves significant advancements in detecting mispronunciations. 

% The integration of articulatory features and auxiliary tasks enhances the distinction between phonemes, while the inclusion of multilingual and monolingual features further improves the accuracy of predicting mispronunciation sequences. This study demonstrates the effectiveness of these combined techniques, pushing the boundaries of existing methods and offering promising prospects for more precise mispronunciation detection.

% This paper presents a novel multi-view multi-task approach for mispronunciation detection, leveraging both multilingual and monolingual pre-trained models in a multi-task setting using articulatory features. 

% By incorporating both articulatory features as auxiliary tasks and leveraging a combination of multilingual and monolingual features, our approach demonstrates significant advancements in mispronunciation detection. 

% The integration of articulatory features auxiliary tasks enhances the distinction between phonemes, while the inclusion of multilingual and monolingual features further augments the accuracy of mispronunciation sequence prediction. 

% This research showcases the effectiveness of these combined techniques, pushing the boundaries of state-of-the-art methods and offering promising prospects for more precise mispronunciation detection.

% Experimental results demonstrate the effectiveness of incorporating articulatory features auxiliary tasks in the mispronunciation detection framework. This research pushes the boundaries of state-of-the-art techniques and contributes to more accurate mispronunciation sequence prediction. 
% In this paper we propose multi-viwe multi-task approach for mispronunication detection , making use of multilingual and monoligual pre-trained models, in amulti task seeting to oreduct ohoneme seuqnce and Articulatory features sequence. The paper introduce the use of articulatory features predictions as auxialary tasks that helps the mispornunication detection models to distinguish between close phoneme those a pushing the state of the art into a more accuracte sequence prediction. We showed also the effectiveness of Articulatory features auxiliary tasks on . 
% Automatic spoken language assessment poses a significant challenge, particularly for second language learners (L2 learners). Mispronunciation detection, the identification of pronunciation errors, stands out as a key challenge. Leveraging articulatory features, which aid in distinguishing phonemes, holds promise for effective mispronunciation detection. In this paper, we propose innovative methodologies for detecting and diagnosing mispronunciations in L2 speech using articulatory features in a multi-task learning (MTL) framework. 
% To accomplish this, we employ the Wav2vec 2.0 model as our acoustic encoder and fine-tune it using L2 speech samples. Our proposed approach encompasses two MTL strategies: (1) C-Wav2vec2.0, employing a cascaded Wav2vec 2.0 model for phoneme sequence recognition and sequences of four articulatory features; and (2) Seq-Wav2vec2.0, employing a sequential learning model for phoneme recognition and articulatory features. To evaluate the effectiveness of our proposed methods, we compare them against baseline approaches on the publicly available L2-Arctic dataset. The experimental results demonstrate that our proposed methods yield substantial improvements in mispronunciation detection and diagnosis. Furthermore, incorporating articulatory features within an MTL framework enhances the performance of our proposed methods. Specifically, our proposed methods achieved phoneme reduction error rates of 11.12\% and 8.23\% respectively, utilizing the two proposed MTL settings. Additionally, we conducted an encoder pruning experiment by removing 2/3 of the encoder layers in the Wav2vec 2.0 model. Remarkably, the pruned model, when coupled with articulatory features, achieved comparable results to state-of-the-art models within the proposed MTL settings. In fact, the pruned model achieved an improvement of 24.22\% and 18.38\% in phoneme reduction error rates, respectively.


% In this study, we propose a MD framework that leverage multi-view representations extracted from both monolingual and multilingual pre-trained speech models, to learn phonetic properties that are: (a) distinct to the target language; and (b) shared across multiple languages. We further disambiguate these phonetic representation by adapting multi-task training with different articulatory feature set classification as an auxiliary task. 

% In this study, we propose a MD framework that leverage multi-view representations extracted from both monolingual and multilingual pre-trained speech models and learn to disambiguate phonetic representation by adapting multi-task training regimen with auxilary tasks. Our approach aims to learn phonetic properties that are: (a) distinct to the target language; and (b) shared across multiple languages. We further disambiguate these phonetic representation by adapting multi-task training with different articulatory feature set classification as an auxiliary task. 




classify quantised values of different articulatory feature sets (AFs). Using this multi-view and multi-task training, the model learns to disentangle fine-grained phonetic properties that are distinct to the target language and shared across multiple languages and .

on distinctive properties of speech production that AFs represent that are distinct to the target language and shared across multiple languages.


based on distinctive properties of speech production that AFs represent 
that are distinct to the target language and shared across multiple languages.

utilizes multi-view representations extracted from both monolingual and multilingual pre-trained speech models. The framework also incorporates multi-task training with auxiliary tasks to disambiguate phonetic representations. The primary objective is to learn phonetic properties that are distinct to the target language and also shared across multiple languages. Additionally, we leverage different articulatory feature set classifications as an auxiliary task to further enhance the disambiguation of these phonetic representations.

Since the articulatory features are the phonological basis of pronunciation (add Browman and Goldstein 1992) and can be used 
We trained the contributors for mispronunciations


multi:  identify phonetic properties that are shared by multiple languages.
% mono: compare the phonetic properties of a language as spoken by different speakers. identify phonetic properties that are influenced by the speaker's native language, the speaker's accent,
identify phonetic properties that would not be visible in either monolingual or multilingual data alone.



, Computer-aided Pronunciation Training (CAPT) has recently gained traction. CAPT systems provide personalized and interactive training to help non-native speakers improve their pronunciation and language skills. Through CAPT, non-native speakers can receive feedback and training tailored to their individual needs, enabling them to overcome the challenges posed by L1-L2 phonological differences.

The phonological differences between a non-native speaker's mother tongue (L1) and the target language (L2) heavily influence their language learning process, leading to segmental errors. To mitigate such errors, there has been a growing interest in the use of self-directed, personalized, and interactive pronunciation training systems, such as Computer-aided Pronunciation Training (CAPT). These systems have gained traction as effective tools for assisting non-native speakers in improving their pronunciation skills and overcoming phonological challenges associated with L2 acquisition.

% Non-native speakers are heavily influenced by their mother tongue (L1) when learning the target language (L2). The difference in phonology between the native and the target language systems of the speakers is one of the main factors for such segmental errors.\footnote{}
% To overcome such errors, self-directed, personalized and interactive pronunciation training systems like Computer-aided pronunciation training (CAPT) has recently gained traction. 

Computer-aided pronunciation training (CAPT) has gained traction for personalized and interactive pronunciation training. One of the goal of CAPT is to facilitate self-directed language learning

where a speaker substitute some phonetic unit (it can be non-existent in the learners’ mother tongue) with the closest one in the mother tongue..
% (Meng, Zee et al. 2007)
In this study, we leverage multiple views (representation) of the acoustic signal to identify phonetic properties shared by multiple languages and compare them to the  
harness the comparitive information encoded  


introduced a multilingual and monolingual pre-trained models within a multi-task framework 
leverage multiple views (representation) of the acoustic signal seen by the pretrained monolinual and multilingual models.
% trained with monolinual and multilingual data respectively. 
These views are extracted

, extracted from monolingual and multilingual pretrained speech models.  to capture a broader range of phonetic representations. 
We opt for multi-view strategy to 
This multiview learning strategy allows for a more comprehensive understanding of pronunciation variations across different languages and dialects.
extracted from monolingual and multilingual pretrained speech models, to capture shared phonetic information between  in the latent space. 








% With the advancement of speech technology, Computer-aided pronunciation training (CAPT) has gained traction for personalized and interactive pronunciation training. One of the goal of CAPT is to facilitate self-directed language learning, detecting 
% both
% supra-segmental (e.g., lexical stress, utterance-level stress, intonation among others) and 
% segmental (e.g., substitution of some phonetic units) errors \cite{}, which is critical for smooth information flow between the speakers. 
% Comparatively, the segmental error is more critical and can greatly harm the information flow between the speakers. 
% The mispronunciation detection (MD) and diagnosis system is a crucial part of the CAPT to detect such segmental errors in an L2 learner's speech and provide effective feedback. 
% Researchers have explored various approaches for evaluating the quality of pronunciation. 
% Over the years, many approaches have been explored. The majority of these approaches rely on pre-trained automatic speech recognition (ASR) systems.

% Over the years, various approaches have been investigated, with the majority relying on pre-trained automatic speech recognition (ASR) systems.
% These methods either (i) identify discrepancies between the aligned ASR output and the reference sequence, or (ii) utilize the log-posterior probability from the ASR to calculate different measures of pronunciation goodness (GOP) scores, as documented in prior works \cite{GOP_WITT, GOP_1, GOP_2}. 
 
% A successful research direction has treated the task of detecting mispronunciations as either a regression or a classification problem \cite{transfer}. Deep learning techniques have been employed in this line of research, with two main approaches. In the first approach, the network is trained end-to-end \cite{non_ASR, non_ASR_2, non_ASR_3, DNN_3}. The second approach involves leveraging computed GOP features from a pre-trained ASR system to build the detection network \cite{JIM, likeJIM_asr, 3M}.




% and the promotion of online learning, computer-aided pronunciation training (CAPT) has been more fully applied to language teaching. As an important part of CAPT technology, mispronunciation detection and diagnosis (MD\&D) can be used to detect the mispronunciation 
% in an L2 learner's speech and provide effective feedback. Researchers have explored various approaches for evaluating the quality of pronunciation. The majority of these approaches rely on pre-trained automatic speech recognition (ASR) systems. These methods either (i) identify discrepancies between the aligned ASR output and the reference sequence, or (ii) utilize the log-posterior probability from the ASR to calculate different measures of pronunciation goodness (GOP) scores, as documented in prior works \cite{GOP_WITT, GOP_1, GOP_2}. 
% \newline




% Currently, most phonetic-level MD systems perform end-to-end phoneme recognition on L2 speech, based on deep neural network (DNN) architectures. The end-to-end structure has demonstrated remarkable effectiveness in ASR tasks yielding promising results in MD \cite{leung2019cnn, feng2020sed, yan2020end, zhang2020end, wu2021transformer, zhang2021text, fu2021full, yan2023peppanet}. Notably, the CNN-RNN-CTC model for free phone recognition, proposed in  \cite{leung2019cnn}, surpasses the performance of previous approaches. Furthermore, a hybrid CTC-Attention architecture was employed, expanding the original L2 phone set with anti-phone set to detect both categorical and non-categorical errors \cite{yan2020end}. These CTC-based methods eliminate the need for forced alignment and seamlessly integrate the entire training pipeline. 

% Various approaches have emerged for mispronunciation detection, capitalizing on the capabilities of acoustic self-supervised encoders such as wav2vec2.0 \cite{baevski2020wav2vec}. An effective methodology involves the utilization of CTC decoding techniques to generate sequences of phonemes for the purpose of mispronunciation detection \cite{xu2021explore, peng2021study},  this approach demonstrates superior outcomes compared to prior research endeavors that solely rely on slef supervised pre-trained models.
% % One notable approach involves employing CTC decoding techniques to generate phoneme sequences for detection purposes \cite{xu2021explore, peng2021study}. 

% Furthermore, a comprehensive approach for mispronunciation detection has been investigated \cite{lin2022phoneme}, involving the integration of frame-level phoneme recognition, textual information, and boundary detection. The study jointly learns to predict the phonemes at the frame level and detect their boundaries by utilizing phoneme sequence embeddings. Frame-level phoneme recognition encompasses the analysis of individual frames of speech data to identify instances of mispronunciation. By incorporating reference text information and boundary detection into the framework, the accuracy of mispronunciation detection at the frame level is significantly improved. This integrated approach allows for more effective and nuanced analysis of mispronunciations, taking into account both phonetic patterns and the specific locations of mispronounced segments within the speech signal.

% Moreover, an alignment method based on articulatory features to align the phone sequences of the reference text with L2 learners’ speech  was proposed \cite{chen2022alignment}. The manner and places of articulation serve as constraints for aligning the reference text with the speech data. This approach incorporates the information from the reference text as additional input, and corresponding articulatory features constraints which helpps avoiding misleading information from reference text.

% Moreover, a recent study by Chen et al. \cite{chen2022alignment} proposed an innovative alignment method that leverages articulatory features to align phone sequences of reference text with L2 learners' speech. This method employs the constraints provided by the manner and places of articulation to facilitate the alignment process between the reference text and the speech data. By incorporating the information from the reference text as additional input, this approach enhances the alignment accuracy. Additionally, the utilization of articulatory feature constraints aids in avoiding the introduction of misleading information from the reference text, thereby ensuring more reliable alignment results.

% Existing methods for mispronunciation detection using self-supervised acoustic models often rely on additional complex textual encoders with additional attention layers to achieve better results, and additional time-alignment that are diffult to obtain. In this paper, we propose a novel approach that uses articulatory features, in a multi-task learning framework. This approach overcomes the limitations of previous methods and achieves substantial improvements in mispronunciation detection and diagnosis. Our experiments show that the proposed approach can achieve comparable results to state-of-the-art models while reducing the number of layers by 2/3, making it more efficient and practical for real-world applications.



% In our study, we leverage both multilingual and monolingual features, and explore a multi-task setting involving phoneme sequence prediction, along with additional task of predicting articulatory features. Our primary motivation for including articulatory features as targets is to enhance the discrimination between phonemes that have similar acoustic representations. To the best of our knowledge, the combination of multilingual and monolingual pretrained model, a multi-view approach, and the inclusion of articulatory features as targets has not been extensively explored in prior studies. This unique combination allows us to capture a broad range of linguistic characteristics and acoustic variations, leading to a more robust and accurate phoneme sequence prediction. 



% With the development of speech technology and the promotion of online learning, computer-aided pronunciation training (CAPT) has been more fully applied to language teaching. As an important part of CAPT technology, mispronunciation detection and diagnosis (MD&D) can be used to detect the mispronunciation in a L2 learner‘s speech, and further diagnose and give learners effective feedback.

% A common feature used for automatic pronunciation as- sessment is GOP, which is defined as the posterior probability of the uttered phoneme given the corresponding acoustic seg- ment [1]. GOP was first computed using Gaussian-mixture- model-hidden-Markov-model-based (GMM-HMM) acoustic models [1], and it has prevailed in the related studies ever since. With the development of the deep neural network (DNN), it has been demonstrated that DNN-HMM- based ASR can reduce word error rate (WER) significantly compared with GMM-HMM models.

% In this study, we focus on detecting phonetic-level pronunciation errors for L2 speech assessment. Currently, most phonetic-level mispronunciation detection and diagnosis (MDD) systems perform end-to-end phoneme recognition on L2 speech, based on deep neural network (DNN) architectures [3, 4, 5, 7, 8]. One of the challenges of training such DNNs is data sparsity, due to the laborious process of annotating perceived phonemes on L2 speech.  To address this issue, the “pre-training + fine-tuning” scheme has been shown to be effective [9]: in pre-training stage a model was trained on external large scale unlabeled data using self-supervised learning (SSL) objectives, and then fine-tuned on the data from the downstream task with task-specific supervision. 


% Recently, pre-training has gained popularity in different areas such as natural language processing (NLP) and speech processing to train models with unlabeled data by unsupervised learning or semi-supervised learning methods. By fine-tuning the pre-trained model, many downstream tasks have achieved excellent performance with limited amounts of labeled data. A pre-trained model called wav2vec 2.0 was proposed, and it has achieved state-of-the-art (SOTA) performance in phoneme recognition by fine-tuning on TIMIT dataset. Wav2vec 2.0 has been successfully applied to mispronunciation detection and diagnosis (MDD) with CTC to decode phoneme sequence. Inspired by these studies, we try to utilize pre-trained models for pronunciation assessment to reduce the need for labeled data, 

